Projective Ranking-based GNN Evasion Attacks

Graph neural networks (GNNs) offer promising learning methods for graph-related tasks. However, GNNs are at risk of adversarial attacks. Two primary limitations of the current evasion attack methods are highlighted: (1) The current GradArgmax ignores the "long-term" benefit of the perturbation. It is faced with zero-gradient and invalid benefit estimates in certain situations. (2) In the reinforcement learning-based attack methods, the learned attack strategies might not be transferable when the attack budget changes. To this end, we first formulate the perturbation space and propose an evaluation framework and the projective ranking method. We aim to learn a powerful attack strategy then adapt it as little as possible to generate adversarial samples under dynamic budget settings. In our method, based on mutual information, we rank and assess the attack benefits of each perturbation for an effective attack strategy. By projecting the strategy, our method dramatically minimizes the cost of learning a new attack strategy when the attack budget changes. In the comparative assessment with GradArgmax and RL-S2V, the results show our method owns high attack performance and effective transferability. The visualization of our method also reveals various attack patterns in the generation of adversarial samples.

==> sections/bio.tex <==
\vspace{-50pt}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{fig/HeZhang.jpg}}]{He Zhang} is currently a Ph.D. student with the Faculty of Information Technology, Monash University, Australia. His research interests include graph neural networks, graph attack and defence, and adversarial deep learning.
\end{IEEEbiography}
\vspace{-50pt}
% \begin{IEEEbiographynophoto}{Xingliang Yuan}
% Biography text here.
% \end{IEEEbiographynophoto}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{fig/XingliangYuan.jpg}}]{Xingliang Yuan} is currently a Senior Lecturer with the Faculty of Information Technology, Monash University, Australia. He obtained his PhD degree in Computer Science from City University of Hong Kong in 2016. His research interests include data security and privacy, machine learning security, secure networked systems, and confidential computing. His research has been supported by Australian Research Council, CSIRO Data61, and Oceania Cyber Security Centre. In the past few years, his work has appeared in prestigious venues in information security, computer networks, and distributed systems, such as ACM CCS, NDSS, IEEE INFOCOM, IEEE TDSC, IEEE TPDS, etc.
\end{IEEEbiography}
\vspace{-50pt}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{fig/Zhou.jpg}}]{Chuan Zhou} obtained the Ph.D. degree from Chinese Academy of Sciences in 2013. He won the outstanding doctoral dissertation of Chinese Academy of Sciences in 2014, the best paper award of ICCS-14, and the best student paper award of IJCNN-17. Currently, he is an Associate Professor at the Academy of Mathematics and Systems Science, Chinese Academy of Sciences. His research interests include social network analysis and graph mining. To date, he has published more than 90 papers, including IEEE TKDE, IEEE TNNLS, IEEE TPAMI, NeurIPS, AAAI, IJCAI, etc.
\end{IEEEbiography}

\vspace{-50pt}
% if you will not have a photo at all:
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{fig/shirui-bio.jpg}}]{Shirui Pan} received a Ph.D. in computer science from the University of Technology Sydney (UTS), Ultimo, NSW, Australia. He is a Professor and an ARC Future Fellow (2021-2025)  with the School of ICT, Griffith University, Australia.
%Prior to this, he was a Lecturer with the School of Software, University of Technology Sydney. 
His research interests include data mining and machine learning. To date, Dr Pan has published extensively in top-tier journals and conferences, including TPAMI, TNNLS, TKDE, ICML, NeurIPS, KDD, AAAI, IJCAI, WWW, CVPR, ACL, and ICDM. %His research has attracted over 8000 citations. 
He is a recipient of the Best Student Paper Award of IEEE ICDM 2020. %His survey paper on \textit{``A Comprehensive Survey on Graph Neural Networks"} in TNNLS-21 has been cited over 2900 times. 
He is recognised as one of the AI 2000 AAAI/IJCAI Most Influential Scholars in Australia (2021). %He is currently
%organizing a special issue, i.e., “\emph{Deep Neural Networks for Graphs:
%Theory, Models, Algorithms and Applications}”, in IEEE TNNLS.%the IEEE Transactions on Neural Networks and Learning Systems (TNNLS), IEEE Transactions on Knowledge and Data Engineering (TKDE),  and KDD.
\end{IEEEbiography}

